Controller Synthesis for Discrete-time Hybrid Polynomial Systems via Occupation Measures

We consider the feedback design for stabilizing a rigid body system by making and breaking multiple contacts with the environment without prespecifying the timing or the number of occurrence of the contacts. We model such a system as a discrete-time hybrid polynomial system, where the state-input space is partitioned into several polytopic regions with each region associated with a different polynomial dynamics equation. Based on the notion of occupation measures, we present a novel controller synthesis approach that solves finite-dimensional semidefinite programs as approximations to an infinite-dimensional linear program to stabilize the system. The optimization formulation is simple and convex, and for any fixed degree of approximations the computational complexity is polynomial in the state and control input dimensions. We illustrate our approach on some robotics examples.

==> sec/examples/0_hybridized_double_integrator.tex <==
\subsection{Hybridized double integrator}
Consider a double integrator discretized by the explicit Euler scheme with a sampling time $\delta t = 0.01$.
The discrete-time dynamics equations are 
\begin{align*}
    &x_1^+ = x_1 + 0.01x_2,\\
    &x_2^+ = x_2 + 0.01u.
\end{align*}

Let the state constraint set be $X = \{x\in \R^2: |x_1|\leq 1, |x_2|\leq 1\}$, and the target set $Z = \{x\in \R^2: |x_1| \leq 0.1,|x_2|\leq 0.1\}$.
We hybridize the system by splitting $X$ at $x_1 = 0.5$, i.e., let $s = 2$, $X_1 = \{x\in \R^2: -1\leq x_1\leq 0.5, |x_2|\leq 1\}$, and $X_2 = \{x\in \R^2: 0.5\leq x_1\leq 1, |x_2|\leq 1\}$.
The dynamics in each mode is the same as given above.
We searched for a degee-1 controller, i.e., a piecewise-affine controller. 
The extracted controller is 
\begin{align*}
    &u^1(x) = -0.079924-1.1147x_1-1.4952x_2, \text{ for } x\in X_1,\\
    &u^2(x) = -0.36197-0.53351x_1-0.6395x_2, \text{ for } x\in X_2.
\end{align*}
We sampled initial states uniformly in $X$ and computed if each initial state can be controlled to the target set under the extracted controller.
In the left plot of Figure \ref{fig:hybrid_double_integrator}, the red dots represent the initial states that can be controlled to the target set under the extracted controller in 1000 time steps, while the blue dots represent those cannot.
The right plot of Figure \ref{fig:hybrid_double_integrator} shows the trajectories of the four initial states, $(0.8,-0.9),(0.4,0.6),(-0.7,-0.8)$, and $(-0.5,0.9)$, under the extracted controller.

\begin{figure}[H]
  \includegraphics[width=.45\linewidth]{pic/hybrid_double_integrator_degree_1_controllable_points_20x20.pdf}
  \includegraphics[width=.45\linewidth]{pic/hybrid_double_integrator_degree_1_4trajs.pdf}
  \caption{Left: The red dots represent the initial states that can be controlled to the target set under the extracted controller in 1000 time steps, while the blue dots represent those cannot. Right: Trajectories of four initial states under the extracted controller. The vertical line at $x_1 = 0.5$ represents the boundary between $X_1$ and $X_2$.}
  \label{fig:hybrid_double_integrator}
\end{figure}


==> sec/examples/1_hybridized_dubins_car.tex <==
\begin{figure}[t]
  \includegraphics[width=.45\linewidth]{pic/hybrid_dubins_car_d8_controllable_points_section1.pdf}
  \includegraphics[width=.45\linewidth]{pic/hybrid_dubins_car_d8_controllable_points_section2.pdf}\\
  \includegraphics[width=.45\linewidth]{pic/hybrid_dubins_car_d8_controllable_points_section3.pdf}
  \includegraphics[width=.45\linewidth]{pic/hybrid_dubins_car_d8_controllable_points_section4.pdf}\\
  \includegraphics[width=.45\linewidth]{pic/hybrid_dubins_car_d8_controllable_points_section5.pdf}
  \includegraphics[width=.45\linewidth]{pic/hybrid_dubins_car_d8_6trajs.pdf}
  \caption{First five plots from top to bottom: Controllable points in five 2D sections at $x_2 = -1, -0.6, 0, 0.6$, and $1$. Bottom right: Six trajectories starting from controllable initial states.}
  \label{fig:dubins_car_grid}
\end{figure}

\subsection{Hybridized Dubin's car}
Consider the Dubin's car model (Example 2 in \cite{han2018controller}).
It is naturally a non-hybrid system and we will hybridize it by splitting its state space into two cells. 
%We use this example to show that our method can cope with hybrid polynomial dynamics instead of simply PWA dynamics.
The dynamics of the Dubin's car model is given by 
\[
    \dot{a} = v\cos(\theta), \dot{b} = v\sin(\theta), \dot{\theta} = \omega,
\]
where $a$ and $b$ are the coordinates in the 2D plane, and $\theta$ is the yaw angle.
The control inputs are the forward velocity $v$ and the angular velocity $\omega$.
By coordinate transformation, the dynamics can be rewritten as
\[
    \dot{x}_1 = u_1, \dot{x}_2 = u_2, \dot{x}_3 = x_2 u_1 - x_1 u_2,
\]
which is also known as the Brockett integrator.
The system has an uncontrollable linearization at any equilibrium and does not admit any continuous time-invariant control law that globally stabilizes the origin \cite{devon2007kinematic}.

Discretize the system using the explicit Euler scheme with a sampling time $\delta t = 0.01$.
Let $X = \{x\in \R^3: ||x||_\infty\leq 1\}$, and $Z = \{x\in \R^3: ||x||_\infty \leq 0.1\}$.
Hybridize the system by setting $s = 2, X_1 = \{x\in \R^3: ||x||_\infty\leq 1, x_2 \leq 0.5\}$, and $X_2 = \{x\in \R^3: ||x||_\infty\leq 1, x_2 \geq 0.5\}$.
The dynamics in two modes are the same.
We searched for a degree-4 hybrid controller.
The computation time on an Intel i7-3960X, 12 core, 3.30 GHz, 32 GB RAM machine was approximately 10 minutes.
We sampled initial states uniformly in $X$ and computed if each initial state can be controlled to the target set under the extracted controller.
In Figure \ref{fig:dubins_car_grid}, the controllable sample states under the extracted controller are plotted as red points in five 2D sections at $x_2 = -1, -0.6, 0, 0.6$, and $1$.
The bottom right plot shows six trajectories starting from the controllable initial states, $(-1,1,0.9)$, $(1,1,0)$, $(-0.2,1,-0.7)$, $(0.7,-1,0.9)$, $(1,-1,-0.6)$, and $(-1,-1,-0.6)$.


==> sec/examples/3_cart_pole_with_a_wall.tex <==
\subsection{Cart pole with a wall}
Consider the problem of balancing the cart-pole system with the existence of a nearby elastic wall, as shown in Figure \ref{fig:cart_pole_with_a_wall_pic}.
The system parameters are $m_c = 1, m_p = 1, l = 1, g = 10, \delta t = 0.01, d = 0.5, k = 50$.
Let $q = [x,\theta]^\top, \mathbf{x} = [q^\top, \dot{q}^\top]^\top$, and $u = f$.
We are interested in controlling the system to its unstable fixed point $\mathbf{x}^* = [0,0,0,0]^\top$, by potentially making and breaking contacts with the wall. 
Since we can only exert horizontal force on the cart, the system is underactuated.

\begin{figure}[b]
  \centering 
  \includegraphics[width=.5\linewidth]{pic/cart_pole_with_a_wall.pdf}
  \caption{Cart pole with an elastic wall.}
  \label{fig:cart_pole_with_a_wall_pic}
\end{figure}


Define $X = \{\mathbf{x}\in \R^4| |\mathbf{x}_1|\leq 1.5,|\mathbf{x}_2| \leq \pi/6, |\mathbf{x}_3| \leq 20, |\mathbf{x}_4|\leq 5 \}$.
Linearize the dynamics in each mode, and define $X_1 = \{\mathbf{x}\in X| x-l\theta \leq -d\}$ and $X_2 = \{\mathbf{x} \in X| x-l\theta \geq -d\}$.
Then we scaled the dynamics so that $X = \{\mathbf{x}\in \R^4| \ ||\mathbf{x}||_\infty \leq 1 \}$ and define $Z = \{\mathbf{x} \in \R^4| \ ||\mathbf{x}||_\infty \leq 0.1\}$.
After extracting a piecewise-affine controller, we uniformly sampled states in the 2D section $\Gamma_{12} = \{\mathbf{x}\in X| \mathbf{x}_3 = \mathbf{x}_4 = 0\}$, and plotted the controllable sample states as red dots in the left plot of Figure \ref{fig:cart_pole_with_a_wall}.
The right plot of Figure \ref{fig:cart_pole_with_a_wall} shows the projections of the trajectories of four initial states, $(-0.5,-0.35,0,0)$, $(-0.5,0,0,0)$, $(-0.75,-0.2,0,0)$, and $(1,-0.55,0,0)$, onto the 2D plane $\Gamma_{12}$.
The inclined line segment represents the boundary of two modes in the scaled coordinate system.
The black framed box in the right plot represents the projection of $Z$ on $\Gamma_{12}$.

\begin{figure}[t]
  \includegraphics[width=.48\linewidth]{pic/cart_pole_with_a_wall_d05_k50_xmax_20_5_grid_40x40.pdf}
  \includegraphics[width=.48\linewidth]{pic/cart_pole_with_a_wall_d05_k50_xmax_20_5_4trajs.pdf}

  \caption{Cart pole with a wall. Left: controllable sampled states in the 2D section $\Gamma_{12}$ in red. Right: projections onto $\Gamma_{12}$ of the trajectories of four initial states. The inclined line segment represents the boundary of two modes in the scaled coordinate system.}
  \label{fig:cart_pole_with_a_wall}
\end{figure}


==> sec/examples/4_box_atlas_single_leg.tex <==
\subsection{Simplified one-legged robot}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{pic/box_atlas_single_leg.pdf}
    \caption{simplified one-legged robot}
    \label{fig:box_atlas_single_leg}
\end{figure}
Let $F_f$ and $F_N$ represent the friction and the normal forces at the foot, respectively.
Let $\overline{F}_N = F_N - m_c g$.
Let $q_b = [x_b,y_b]^\top$ and $q_f = [x_f,y_f]^\top$ be the general coordinates of the body and the foot, respectively.
We assume the contact model is the spring-mass model.
The system can be described by the following dynamics equations and constraints:
\begin{align*}
    &\ddot{q}_f - \ddot{q}_b = u,\\
    &\ddot{q}_b = (F_f+\overline{F}_N)/m_c,\\
    &F_f = -k_1\dot{x}_f,\\
    &\overline{F}_N =\begin{cases} -k_2 y_f, \quad \text{if foot in contact with ground,} \\ -m_c g, \quad \text{if foot not in contact,} \end{cases}\\
    &|F_f| \leq \mu F_N.
\end{align*}
Since we do not care about the horizontal position of the leg, we can remove $x_b$ and $x_f$ in the system state, and the system can be described by four states $[y_b,\dot{x}_b,\dot{y}_b,y_f]^\top$.
The control input $u$ can be decomposed as horizontal and vertical inputs and hence is 2-dimensional.
The resulting system is a PWA system with 2 modes.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\linewidth]{pic/box_atlas_single_leg_d1_x1_x4.pdf}
    \includegraphics[width=0.45\linewidth]{pic/box_atlas_single_leg_d1_x2_x4.pdf}
    \includegraphics[width=0.45\linewidth]{pic/box_atlas_single_leg_d1_x3_x4.pdf}
    \caption{Simplified one-legged robot}
    \label{fig:box_atlas_single_leg}
\end{figure}

==> sec/relatex_work.tex <==
The motivation for our study is to design feedback controllers that can stabilize rigid body systems by making and breaking multiple contacts with the environment.
